Poly-Autoregressive Prediction for Modeling Interactions

We introduce a simple framework for predicting the behavior of an agent in multi-agent settings. In contrast to autoregressive (AR) tasks, such as language processing, our focus is on scenarios with multiple agents whose interactions are shaped by physical constraints and internal motivations. To this end, we propose Poly-Autoregressive (PAR) modeling, which forecasts an ego agent's future behavior by reasoning about the ego agent's state history and the past and current states of other interacting agents. At its core, PAR represents the behavior of all agents as a sequence of tokens, each representing an agent's state at a specific timestep. With minimal data pre-processing changes, we show that PAR can be applied to three different problems: human action forecasting in social situations, trajectory prediction for autonomous vehicles, and object pose forecasting during hand-object interaction. Using a small proof-of-concept transformer backbone, PAR outperforms AR across these three scenarios. The project website can be found at https://neerja.me/PAR/.

==> _CVPR_2025__PAR__1_/preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

% checkmarks
\usepackage{pifont}
\newcommand{\cmark}{\textcolor{green!80!black}{\ding{51}}}
\newcommand{\xmark}{\textcolor{red}{\ding{55}}}


\newcommand{\shiry}[1]{{\color{teal}[shiry: #1]}}
\newcommand{\neerja}[1]{{\color{purple}[neerja: #1]}}
\newcommand{\tara}[1]{{\color{orange}[tara: #1]}}
\newcommand{\jathushan}[1]{{\color{blue}[jathushan: #1]}}


==> _CVPR_2025__PAR__1_/sec/0_abstract.tex <==
\begin{abstract}
We introduce a simple framework for predicting the behavior of an agent in multi-agent settings. In contrast to autoregressive (AR) tasks, such as language processing, our focus is on scenarios with multiple agents whose interactions are shaped by physical constraints and internal motivations. To this end, we propose Poly-Autoregressive (PAR) modeling, which forecasts an ego agent’s future behavior by reasoning about the ego agent’s state history and the past and current states of other interacting agents. At its core, PAR represents the behavior of all agents as a sequence of tokens, each representing an agent’s state at a specific timestep. With minimal data pre-processing changes, we show that PAR can be applied to three different problems: human action forecasting in social situations, trajectory prediction for autonomous vehicles, and object pose forecasting during hand-object interaction. Using a small proof-of-concept transformer backbone, PAR outperforms AR across these three scenarios. 
\end{abstract}

==> _CVPR_2025__PAR__1_/sec/1_intro_v2.tex <==
\section{Introduction}

Large language models (LLMs) have been very successful with natural language processing (NLP) tasks, which require accurate reasoning over relationships words have within a body of text. A key component of LLMs is autoregressive (AR) modeling, where each word token is predicted based on a sequence of preceding word tokens. Building on the success of AR modeling in the NLP community, this work focuses on modeling the dynamic relationships between agents and entities in everyday interactions that occur in the physical world, such as social interactions, driving, and hand-object interactions.

Unlike language which is structured through grammar and semantics, interactions in the physical world are dictated by both the laws of physics (\textit{e.g.} how a hand grasps an object) and the internal state of each agent (\textit{e.g.} the trajectory an agent chooses to move a grasped object in) , a latent variable that we know nothing about. Furthermore, as opposed to text where each word follows another unidimensionally, the states of multiple agents are changing simultaneously. For example, in social situations, the history of a single person’s past states does not alone determine the dynamics of their future states; we also need to consider the states of other agents. We argue, therefore, that AR modeling alone is insufficient. 

In this paper, we introduce poly-autoregressive (PAR) modeling, a simple unifying approach to model the influence of other agents and entities on one’s behavior. We model behavior as a temporal sequence of states and predict an ego agent’s future behavior conditioned on the history of behavior of the ego agent as well as the rest of the agents. By considering other agents’ behaviors, we demonstrate that our approach significantly improves upon the ill-posed problem of single-agent prediction in interactive settings.

The PAR framework uses a transformer-based model for next-token prediction. Transformers have shown great success in language modeling and naturally lend themselves to predicting behavior over time. In an  interaction scenario of $N$ agents, our model predicts the future behavior of an ego ($N^{\text{th}}$) agent conditioned on its past behavior and the behavior of the other $N-1$ non-ego agents (see Figure~\ref{fig:polyauto}b). 
Each prediction task may model a different behavior modality of interest, e.g. actions for social action prediction, or 6DoF pose for object forecasting in hand-object interactions. We apply PAR to three different case studies of common real-world interactions: 
 \begin{enumerate}
     \item  \textbf{Social action prediction.} We test our method on the AVA benchmark~\cite{gu2018ava} for action forecasting. By incorporating both the ego and another agent using PAR, we get a overall $+1.9$ absolute mAP gain over AR, which only models the ego agent to predict its future behavior, and an absolute $+3.5$ mAP gain on 2-person interaction classes.
     \item \textbf{Trajectory prediction for autonomous vehicles.} When forecasting future $xy$ locations of an ego vehicle, incorporating the locations of neighboring vehicles with PAR outperforms AR, which only uses the ego vehicle's preceding trajectory as input. Specifically, on the nuScenes dataset~\cite{nuscenes}, PAR outperforms AR with a relative improvement of $6.3\%$ ADE and $6.4\%$ FDE. 
     \item \textbf{6DoF object pose forecasting during hand-object interaction.} We use the DexYCB dataset~\cite{chao2021dexycb}, where we treat the object as the ego agent and the hand as the interacting agent. While PAR integrates that hand's 3D location and object pose history, AR only uses the object's pose history to predict the object's 6DoF pose. PAR outperforms AR with relative improvements of $8.9\%$ and $41.0\%$ for the rotation and translation predictions, respectively.
 \end{enumerate}

In all these settings, we find that incorporating the behavior of other agents in the scene improves predictions of the ego agent's behavior.
All of these problems are modeled via the same simple PAR framework and implemented using the same proof-of-concept 4 million parameter transformer \textit{without any modifications to the base framework or architecture}, only to data pre-processing and choice of tokenization. We also provide an example of a simple way to build on our architecture through a location positional encoding, Sec.~\ref{sec:car_trajs}
.

The primary contribution of this work is a versatile framework that can be applied to a diverse range of settings, without modifications aside from domain-specific data processing. Our results suggest that PAR provides a simple formulation that, with a more complex transformer backbone and larger datasets, could enhance prediction of diverse multi-agent interactions across various problem domains. To facilitate further exploration and development, we have released our code, which contains the building blocks to use PAR for modeling other types of multi-agent interactions.


==> _CVPR_2025__PAR__1_/sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> _CVPR_2025__PAR__1_/sec/2_related_work.tex <==
\section{Related Work}

% 1951 Shannon’s language paper proposing AR modeling~\citep{shannon1951prediction}

% Some informational aspects of visual perception~\citep{attneave1954some}

% Autoregressive models~\citep{larochelle2011neural}


% In deep learning with continuous values~\citep{gregor2014deep,theis2015generative}

% With discrete tokens using a using a
% multinomial distribution~\citep{van2016pixel}

% Massive success in language modeling 
% % \shiry{cite GPT and friends}
% GPT1:~\citep{radford2018improving}

% Then move towards multimodal - Flamingo~\citep{alayrac2022flamingo} etc


\textbf{Autoregressive models.} Autoregressive modeling has a rich history in information theory and deep learning, tracing back to Shannon's paper on language prediction~\citep{shannon1951prediction} and Attneave's study on visual perception~\citep{attneave1954some}. These foundational works laid the groundwork for modern applications in deep learning, including~\citep{larochelle2011neural}, which revisits neural autoregressive models and ~\citep{gregor2014deep, theis2015generative}, which explore continuous-valued modeling. ~\citep{van2016pixel} developed PixelRNN and PixelCNN to autoregressively generate images one pixel at a time using RNN and CNN architectures, respectively. 

\medskip
The development of the transformer model~\citep{vaswani2017attention} spurred progress in computer vision with the image transformer~\citep{parmar2018imagetransformer} and the vision transformer~\citep{dosovitskiy2020image}, and autoregressive models ~\cite{chen2020generative, rajasegaran2025empirical} and more notably in NLP, where the GPT family of models~\citep{radford2018improving, radford2019language, brown2020language} has demonstrated the power of large-scale unsupervised autoregressive pre-training. Recent research has focused on multimodal learning, exemplified by the Flamingo~\citep{alayrac2022flamingo} or LlaVa~\citep{liu2023improved} models, which combine vision and language processing capabilities, illustrating the versatility of autoregressive models across various domains in artificial intelligence. While these approaches operate on image patches and word tokens, we operate on symbolic representations extracted from in-the-wild videos showing natural interactions.  A recent approach~\citep{radosavovic2024humanoid} frames humanoid locomotion as an autoregressive next-token prediction task that operates on two types of continuous tokens: observations and actions. This approach projects continuous tokens to the hidden dimension and uses a shifted loss, similar to the next-timestep prediction proposed in our framework.
% \neerja{add more multimodal examples?}


\medskip
\noindent
\textbf{Multi-agent regressive models.} 
Several prior works addressed modeling specific multi-agent problems via regressive models as one-off case studies. We introduce the PAR framework to unify these efforts into a single cohesive framework. Many behavior prediction works focus on two agents engaging in social interaction, whether it be dyadic communication~\citep{Ng_2022_CVPR, ng2023text2listen, ng2024audio2photoreal} or social dance~\citep{siyao2024duolando,maluleke2024synergy}. These studies primarily tackle the challenge of predicting the state of an interacting partner (Person B) based on the input from Person A's state, sometimes extending predictions into the future~\citep{guo2022multi,maluleke2024synergy}. While earlier works used architectures such as variational RNNs~\citep{baruah2020multimodal}, recent works have predominantly adopted transformer architectures for social interaction modeling~\citep{guo2022multi,Ng_2022_CVPR, 10036100, ng2023text2listen, siyao2024duolando}, with some works exploring diffusion~\citep{liang2024intergen}, or diffusion with attention~\citep{ghosh2024remos}. Our PAR framework focuses on transformer models.

\medskip
Works encompassed by the PAR framework extend beyond human social interaction. Many multi-agent human or car trajectory prediction approaches use autoregressive prediction.  For instance, MotionLM~\citep{seff2023motionlm} utilizes a transformer decoder that processes multi-agent tokens, incorporating a learned agent ID embedding. This methodology informs our approach across all our case studies. \textit{Critically, in contrast to all prior multi-agent regressive works that designed solutions to address specific applications, we demonstrate that we can unify a diverse set of multi-agent regressive problems under a single PAR framework.} See Appendix Sec.~\ref{sec:case_study_related} for case-study-specific works.

% Ilija paper that uses the PAR next timestep prediction for humanoid next token pred~\citep{radosavovic2024humanoid}
% Dyadic communication - Evonne Learning to Listen~\citep{Ng_2022_CVPR}, L2L follow up~\citep{ng2023text2listen}, Audio to Photoreal~\citep{ng2024audio2photoreal}

% Vongani dance paper~\citep{maluleke2024synergy}

% Motion InterGen~\citep{liang2024intergen} diffusion based, only two people in interaction. In contrast, we can model an arbitrary number of people. \shiry{this one is diffusion, not AR - shiry check. Can mention but just to differentiate.}

% \shiry{Need to go over the related work from Vongani's paper to make sure we aren't missing anything that is not specifically dance... like this \url{https://arxiv.org/abs/2403.18811}}

% papers in Lea table:

% A Multimodal Predictive Agent Model for Human Interaction Generation (CVPR-W 2020)~\citep{baruah2020multimodal}: variational RNN w attention, predict agent B given agent A and then predict into the future 

% ReMoS: 3D Motion-Conditioned Reaction
% Synthesis for Two-Person Interactions (ECCV 2024)~\citep{ghosh2024remos}: diffusion + cross-modal attention, predict agent B given agent A

% Duolando (ICLR 2024)~\citep{siyao2024duolando}: uses GPT transformer model AR next token prediction + RL, given music + person A dance, predict/generate person B dance


% InterFormer (2023)~\citep{10036100}: transformer encoder-decoder, given person A pose predict person B  pose

% ExPI (CVPR 2022)~\citep{guo2022multi}: sort of transformer? (cross-interaction
% attention modules); 


% Waymo MotionLM~\citep{seff2023motionlm} \neerja{We are basically implementing a stripped down/simpler version of this paper but showing that their agent ID embedding and next timestep prediction helps on different tasks - so there is some subtlety on how we actually mention this paper}



\medskip
\noindent


==> _CVPR_2025__PAR__1_/sec/3_PAR.tex <==

\begin{figure*}
\centering
    \includegraphics[width=.99\textwidth]{fig/par_method.pdf}  
    \caption{\textbf{The PAR Framework}. We begin by collecting a video dataset, such as AVA (top) or DexYCB (bottom). Then, using dataset labels or computer vision techniques, a trajectory of a given modality for our prediction task is extracted for each agent, such as action class labels (top) or object pose and 3D hand translation (bottom). Data is then tokenized, either through discretization or directly using continuous values, with our framework supporting both formats. Based on the tokenization and prediction task, we choose the appropriate loss function for PAR training. After training with PAR, predicted tokens can be decoded back to data space and evaluated with relevant metrics.}
    \label{fig:PAR_pipeline}
\vspace{-1em}
\end{figure*}

\section{Poly-Autoregressive Modeling}

Our goal is to model the behavior of an agent or entity while taking into account any other agents it interacts  with, if any. To evaluate the performance of our model in capturing interaction dynamics, we predict the agent's future behavior and compare it against ground-truth data. 

We define the following task: \textit{In an interaction comprised of $N$ agents, given the observed past states of the $N-1$ interacting agents, and the observed or previously-predicted past states of the $N^{\text{th}}$ ego agent, predict the future states of the $N^{\text{th}}$  ego agent.}

We define a transformer-based poly-autoregressive (PAR) predictor, $\mathcal{P}$, that learns to model temporally long-range interactions in the input sequence. The inputs to the predictor are the past states of the $N$ interacting agents, and its output is the predicted future state of the $N^{\text{th}}$ ego agent.

\subsection{Problem Definition}
\label{sec:prob_def}

Let $\mathbf{S}=\{\mathbf{s}_i\}_{i=1}^T$ be a temporal sequence of agent states, $\mathbf{s}_i$.
We use $\mathbf{S}^N$ and $\mathbf{S}^{1:N-1}$ to denote the temporal sequences of states of the $N_{th}$ agent and of the other $N-1$ agents, respectively.
For each timestep $t \in [t_\pi,T]$, where $t_\pi \in [1,T]$ is the time we start predicting,
we take as input all other $N-1$ agents' past observed state sequences
$\mathbf{S}^{1:N-1}_{1:t-1}$
along with the $N_{th}$ agent's
past observed states up to $t_\pi$, 
$\mathbf{{S}}^N_{1:t_\pi}$,
and any of its previously predicted past states $\mathbf{\hat{S}}^N_{t_{\pi}+1:t-1}$,
if available (see Fig.~\ref{fig:polyauto}).
Our predictor, $\mathcal{P}$, then \textit{poly-autoregressively} predicts the $N_{th}$ agent's future states one time-step at a time:
\begin{equation}
       \mathbf{\hat{s}}^N_{t} = \mathcal{P}(\mathbf{S}^{1:N-1}_{1:t-1}, \mathbf{{S}}^N_{1:t_{\pi}},\mathbf{\hat{S}}^N_{t_\pi+1:t-1}). \\
\end{equation}
$\mathcal{P}$ learns to model the distribution over the next timestep of the $N_{th}$ agent's states, given all other agents' states:
\begin{equation}
p(\mathbf{\hat{s}}^N_{t} | \mathbf{S}^{1:N-1}_{1:t-1}, \mathbf{S}^N_{1:t-1}).
\end{equation}

While we provide the observed ground truth states of other agents at inference, during training, we jointly maximize the likelihood of all $N$ agents by computing losses on their future state predictions.

We train the predictor by maximizing the likelihood of the target state $y$ at time $t$:
\begin{equation*}
\label{eq:transformerloss}
    \mathscr{L_\mathcal{P}} = E_{y \sim p(y)}[-\log(p(\mathbf{s}^N_{t})],
\end{equation*}
where the target state $y$ at $t$ is computed from the $N_{th}$ agent ground truth future state.

\subsection{The Poly-Autoregressive Framework}
\label{sec:framework}

\begin{figure}
    \centering
    % \begin{subfigure}[b]{0.49\textwidth}
    %     \includegraphics[width=\textwidth]{fig/nexttoken_teacherforcing.pdf}
    %     \caption{AR: next-token training.}
    %     \label{fig:AR_nexttoken}
    % \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{fig/mutli-agent_next-token.pdf}
        \caption{AR: multi-agent, next-token training.}
        \label{fig:AR_multiagent_nexttoken}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{fig/next_timestep.pdf}
        \caption{PAR: same-agent, next-timestep training.}
        \label{fig:PAR_nexttimestep}
    \end{subfigure}    
    \caption{Training with teacher forcing for (a) multi-agent next-token prediction in autoregressive models and (b) multi-agent poly-autoregressive models. Solid vs striped indicates a ground-truth vs predicted token, respectively. Color denotes agent identity. The AR model is trained for next-token prediction, while the PAR model is trained to predict the next timestep of the same agent. Three agents are shown for ease of visualization, but the PAR model supports an arbitrary number of agents.}
    \label{fig:PAR_training}
\vspace{-.75cm}
\end{figure}

We address the problem of forecasting the future states of an agent (from time $t$ to $T$) in a data-driven way, given a temporal sequence of past states (from time $1$ to $t-1$). 
We assume that our agent has some feature, or a set of features, of interest in a video (e.g., 3D pose) that we can tokenize. We predict the future states of the agent in terms of this tokenized feature (or set of), where we use one token (or set of tokens) per time step. The predicted tokens can be discrete (i.e., an index into a feature codebook) or continuous (i.e., a vector of one or more continuous values). The loss $\ell$ will depend on the problem's specifics and the type of token used. To train the model to predict the future, we rely on all the interaction dynamics of length $T$ in our training dataset as ground truth examples.


As a baseline, we consider the \textbf{single-agent autoregressive (AR)} paradigm, where a transformer is trained to perform next-token-prediction with teacher forcing. AR uses greedy sampling to generate sequences at inference time, predicting one next token at a time (Fig.~\ref{fig:polyauto}(a)). 

In contrast, our \textbf{multi-agent poly-autoregressive (PAR)} framework considers the other $N-1$ agents in the scene when predicting the future state of the $Nth$ agent. In this setup, we tokenize the features of interest of all $N$ agents, yielding $N$ tokens at each timestep for a total of $N*T$ tokens. In practice, we operate on a flattened sequence of $N*T$ tokens. 
% In cases where we consider a multimodal set of tokens of interest, we have $T*N*K$ where $K$ is the number of token types. \neerja{The only case where we have multiple token types is hand-object, but there we treat the hand as one agent and the object as another (or equivalently: 1 agent and 2 token types), but regardless $N*K=2$, so we haven't shown $N>1$ and $K>1$} \shiry{ok then we keep this for future ;-) }
Instead of using the AR training procedure in this multi-agent case (as in Fig.~\ref{fig:AR_multiagent_nexttoken}), we jointly model the $N$ agents at each timestep by introducing the following features to our PAR framework.

\vspace{0.2cm}
\noindent \textbf{Next-timestep prediction.} 
A standard AR model predicts the next token. Given the flattened sequence of $N*T$ tokens our model operates on, next token prediction would take as input an agent $k$ at timestep $t$ and predict agent $k+1$'s state at the same timestep $t$ (as in Fig.~\ref{fig:AR_multiagent_nexttoken}). However, our goal is to predict the input agent $k$'s future state at time $t+1$. Therefore, we perform \textit{same-agent next-timestep} prediction rather than next-token prediction (see Fig.~\ref{fig:PAR_nexttimestep} for an illustration of same-agent next-timestep at training).

\medskip \noindent \textbf{Learned agent identity embedding.} When giving a model information corresponding to multiple agents, the model can benefit from knowing which token corresponds to which agent. We give the model this information with a learned agent ID embedding. 
 


 % \medskip \noindent \textbf{Multimodality} \neerja{We have multimodality in the sense of hand and object are different modalities, and we add location to accl/velocity tokens in a pos emb - we should mention that we go beyond just one single type of token per case study, but we also do things in different ways for different case studies so not sure what is the best way to mention this here}


\medskip \noindent \textbf{Joint training.} We train the model to jointly predict the future of all agents by computing a loss on the predicted tokens of all agents (Fig.~\ref{fig:PAR_nexttimestep}). Please refer to Section~\ref{sec:prob_def} for our inference paradigm.

\subsection{Task-Specific Considerations}
\label{sec:task-specific}
Our simple PAR approach unifies diverse problems under a single framework and architecture without any modifications. In order to formulate a problem as interaction-conditioned prediction, users must consider several task-specific details. Fig.~\ref{fig:PAR_pipeline} gives an overview of how the PAR framework disentangles multi-agent learning from problem-specific modeling.

\medskip \noindent \textbf{Data.} The input data source in our example tasks is always a collection of videos. From these videos, we extract various modalities relevant to the task at hand. These modalities can range from high-level features, such as action class labels, to low-level ones, such as 3D pose (Fig.~\ref{fig:PAR_pipeline} first two columns). We assume that each agent in the dataset is detected at each frame and is associated with an agent ID.
 
\medskip \noindent \textbf{Tokenization.} Our framework supports both discrete, quantized tokens and continuous vector tokens. The choice between discrete and continuous depends on the nature of the task.  
In the case of discrete tokens, we use a standard embedding layer to project to the hidden dimension. For continuous tokens, we train a projection layer to project the token into the hidden dimension of the transformer. For instance, if our continuous token is a 3D vector with an $(x,y,z)$ 3D location coordinate and our hidden dimension is $128$, our projection layer will project from $3$ to $128$ dimensions. We also train an un-projection layer that reverts the hidden dimension to the original token dimension.

\medskip \noindent \textbf{Loss.} The type of token and task-specific considerations dictate the loss function $\ell$ applied during model training. For discrete tokens, a classification loss is appropriate. For continuous tokens, we use a regression loss on the original token dimension. 
% \shiry{there is a nuance here that we did not yet have time to explore given the last-minute nature of how this came together: the discrete classification loss allows us to predict a multinomial distribution over possible future timesteps, from which we can sample. This makes the prediction non-deterministic, capturing the true variability of the response of the $N_th$ agent to their surroundings. After all, given other people's actions, our actions are still not determined 100 percent. This is the whole beauty of using autoregressive prediction for these problems, unlike the feed-forward UNets we used in e.g. speech to getsture. This is not at all explored yet in our experiments due to lack of time mostly, and is a major hole in this submission (unlike our previous works on this direction). If a reviewer is familiar with the literature, they will complain about this (I know I would). There is nothing for us to do about this now, but this is something we should be aware of.} \neerja{Adding sampling is high on my priority list!} \shiry{yes, I would reject you without ;-) }

\medskip \noindent \textbf{Baselines.}
We compare to the following baselines, where applicable on a case-by-case basis:

\noindent $\sbullet$ \textit{Random token}: pick random tokens from the best available token space and use as the prediction. 

\noindent $\sbullet$ \textit{Random trajectory}: pick at random a trajectory from the training dataset to use as the prediction. 

\noindent $\sbullet$ \textit{NN}: Given an input agent $A$'s trajectory history, find the closest trajectory to it in the training set, belonging to $A^T$. Use $A^T$'s future as the predicted future.

\noindent $\sbullet$ \textit{Multiagent NN}: In a dataset with two interacting partners $A$ and $B$, where $B$ is the ego agent, given an input agent $A$'s trajectory history, find the closest trajectory to it in the training set, belonging to $A^T$. Use $A^T$'s interaction partner's $B^T$'s future as the prediction.

% Assume two agents, $A$ and $B$ in interaction, where we are predicting agent $B$. Take the history of agent $A^V$ in the validation set and find the closest $A^T$ in the training dataset. Use the future of the corresponding interacting agent $B_T$ in the training trajectory as the predicted future for agent $B_V$.

\smallskip
\noindent $\sbullet$ \textit{Mirror}: In a dataset with two interacting partners $A$ and $B$, use the ground truth future of agent $B$ as the predicted future for agent $A$.



\subsection{Framework Implementation Details}
We keep the following implementation details constant for all case studies (see also Sec.~\ref{sec:appendix_impl_details}).

\medskip
\noindent \textbf{Learned agent ID embedding.} Our learned agent ID embedding consists of the integer agent ID mapped to a hidden dim-sized vector, and summed to the token embedding.

\medskip \noindent \textbf{Architecture.} For all case studies, we use the  Llama~\citep{touvron2023llamaopenefficientfoundation} transformer decoder architecture with $8$ layers, $8$ attention heads, and a hidden and intermediate dimension of $128$. The decoder has $\sim$4.4M learned parameters, not including learned embedding layers which add a few thousand more parameters. A rotary positional encoding~\citep{su2024roformer} is used in addition to other summed encodings (i.e. agent ID embedding, locational positional encoding in Sec.~\ref{sec:car_trajs}). We train using teacher forcing. The only hyperparameter that changes between case studies is the learning rate.


==> _CVPR_2025__PAR__1_/sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> _CVPR_2025__PAR__1_/sec/4_AVA_action_pred.tex <==
\section{Case Study 1: Social Action Forecasting}

\begin{figure*}[t]
    \centering
    \includegraphics[width=.9\textwidth]{fig/ava_qual.pdf}
    \caption{\textbf{Action forecasting example.} The distribution over ground truth actions are in white, and our predictions in red. A 6s action history (1Hz) is input, and 6s of future actions predicted. In the scene, the man and woman alternate between talking and listening. Initially, the man is talking. The AR model predicts he will continue talking, while the 2-agent PAR model recognizes the woman is talking and predicts more accurate turn-taking behavior.}
    \label{fig:ava_qual}
    \vspace{-.6cm}
\end{figure*}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/specified_classes_comparison.pdf}
    \small
    \caption{\textbf{Per-class mAP for AVA 2-person actions}. We see performance improvement on almost all 2-person AVA action classes ((P) stands for ``a person"). Some absolute mAP gains are particularly significant: \textit{listen to} $+7.0$, \textit{kiss} $+8.3$, \textit{fight/hit} $+5.7$, \textit{talk to} $+4.4$, \textit{hug} $+5.7$, and
    \textit{hand shake} $+4.0$.}
\label{fig:ava_2_person_classes}
\vspace{-.5cm}
% \end{wrapfigure}
\end{figure}

Our first case study involves forecasting human actions. Human behaviors are fundamentally social; for instance, individuals frequently walk in groups and alternate between speaking and listening roles when conversing. Certain actions, like hugging or handshaking, are intrinsically multi-person. Therefore, modeling human interactions should help improve action forecasting performance, especially on multi-person actions, which we show in this case study.


\subsection{Experimental Setup}
\noindent \textbf{Dataset.}  The Atomic Visual Actions (AVA) dataset~\citep{gu2018ava} comprises 235 training and 64 15-minute validation videos from movies. Annotations are provided at a 1Hz frequency, detailing bounding boxes and tracks for individuals within the frame, and each person's actions within a 1-second timeframe. Individuals may engage in multiple concurrent actions from a repertoire of 60 distinct action classes (e.g., sitting and talking simultaneously). For our analysis, we select clips featuring a continuous sequence of an agent's actions spanning at least $4$s, splitting sequences exceeding $12$s.  We use the first half of each clip as history to predict the second half. For any ego agent trajectory, we pick a second agent by selecting the person present in the scene for the longest subset of the ego agent's trajectory.

% \medskip \noindent \textbf{Tokenization.}
\medskip \noindent \textbf{Task-specific considerations.} Each agent's token $\mathcal{A}$ represents an 60-dimensional vector that corresponds to the actions performed at a specific timestep. Each element denotes the probability of a particular action class being enacted; ground-truth inputs are a binary vector. We implement an embedding layer that projects these tokens into the transformer's hidden dimension, as well as an un-projection layer that reverts them back to the original 60D token space for the purposes of loss calculation and output generation. We do not explicitly require the outputs to be values between 0 and 1.
% \medskip \noindent \textbf{Loss.} 
We use a MSE regression loss on the 60D action tokens: $\mathscr{L} = \frac{1}{n} \sum_{i=1}^{n} (\mathcal{A}_i - \hat{\mathcal{A}}_i)^2$.
% \medskip \noindent \textbf{Metrics.} 
Our evaluation metric is the
% We measure 
mean average precision (mAP) on the 60 AVA classes.

We implement all baselines described in \ref{sec:task-specific}, where \textit{Random Token} corresponds to a random 60D vector sampled from 0 to 1. \textit{NN} and \textit{Multiagent NN} use Hamming distance as the distance metric.
\begin{table}
% 
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
Method & Timestep pred & Ag-ID embd & mAP $\uparrow$           \\
\midrule
1-agent AR   & N/A         & N/A        & 40.7        \\
2-agent AR   & \xmark      & \xmark     & 38.0      \\
2-agent PAR*  & \xmark     & \cmark     & 40.2         \\
2-agent PAR*   & \cmark     & \xmark   & 40.0         \\
2-agent PAR &\cmark  & \cmark & \textbf{42.6}     \\
\bottomrule
\end{tabular}
\caption{\textbf{PAR action forecasting performance on AVA} We evaluate 1 and 2-agent AR methods, two 2-agent PAR ablations (rows 3 and 4, PAR*), and our PAR method. Without next-timestep prediction (see Fig.~\ref{fig:PAR_training}) or a learned agent ID embedding, our model struggles with multi-agent reasoning, performing worse than the AR baseline. With both components, the 2-agent PAR model achieves a +1.9 mAP gain over the AR method (see Fig.~\ref{fig:ava_1_person_classes} and Fig.~\ref{fig:ava_2_person_classes} for class breakdown).}
\label{tab:ava_PAR_ablation}
\vspace{-.25cm}
\end{table}
% neerja: experiment names and wandb links
% 1-agent	https://wandb.ai/nthakkar/PAR_ava_action_prediction_post_ICLR/runs/s9sa5w5o?nw=nwusernthakkar	action_pred_ava_1_agent_lr_5e-5_ema_decay_0.999_seed_1_val_full_val
% 2-agent AR	https://wandb.ai/nthakkar/PAR_ava_action_prediction_post_ICLR/runs/nh9gvjlu?nw=nwusernthakkar	action_pred_ava_2_agent_no_ag_id_emb_no_same_ag_loss_lr_5e-5_ema_decay_0.999_seed_1_val_full_val
% 2-agent no timestep pred	https://wandb.ai/nthakkar/PAR_ava_action_prediction_post_ICLR/runs/xzlllmta	action_pred_ava_2_agent_no_same_ag_loss_lr_5e-5_ema_decay_0.999_seed_1_val_full_val_vis
% 2-agent no ag id emb	https://wandb.ai/nthakkar/PAR_ava_action_prediction_post_ICLR/runs/3uzemj2m?nw=nwusernthakkar	action_pred_ava_2_agent_no_ag_id_emb_lr_5e-5_ema_decay_0.999_seed_1_val_full_val_vis
% 2-agent PAR	https://wandb.ai/nthakkar/PAR_ava_action_prediction_post_ICLR/runs/u5yoe6vs?nw=nwusernthakkar	actual_final_ava_1hz_action_2_agent_ag_id_emb_full_val_val_full_val
% https://wandb.ai/nthakkar/PAR_ava_action_prediction/runs/ramhpxe1?nw=nwusernthakkar	
\begin{table}
% 
\centering
\begin{tabular}{@{}lcc@{}}
\toprule
Baseline & Agents &  mAP $\uparrow$           \\
\midrule
Random Token         & 1 & 3.46          \\
Random Training Traj  & 1   & 3.44          \\
Nearest Neighbor    & 1        & 13.17 \\
Multiagent NN &2      & 5.10      \\
Mirror   & 2 & 7.97         \\
\bottomrule
\end{tabular}
\caption{\textbf{AVA baselines} While the nearest neighbor baseline performs best among baselines, it is still significantly worse than the AR model.}
\label{tab:ava_baselines}
\vspace{-.5cm}
\end{table}

\subsection{Results}

We report the performance of a single-agent AR model as a baseline, in the first line of Table~\ref{tab:ava_PAR_ablation}. The AR model is significantly better than our baselines (see Table~\ref{tab:ava_baselines}), the strongest baseline being the single-agent NN. We compare these baselines to our 2-agent PAR model (last line) and various ablations where we remove the agent ID embedding and perform next-token rather than same-agent next-timestep prediction. The second line of the table corresponds to multi-agent next-token prediction (Fig.~\ref{fig:AR_multiagent_nexttoken}). We see that this approach confuses the model, and the performance is significantly worse than just training on and considering a single agent. However, as we add various components of our PAR approach, the performance improves, and with both the next timestep prediction and agent ID embedding, we get a $+1.9$ mAP gain. When only considering 2-person action classes (enumerated in Fig.~\ref{fig:ava_2_person_classes}), our mAP is  $36.3$ on the single agent PAR model and $39.8$ on the 2-agent PAR model, a \textbf{$+3.5$} mAP gain.

In Fig.~\ref{fig:ava_qual} we see an example of action forecasting. In the input history, the man talks and the woman listens. In the future, the woman talks, and the man listens. Our 2-agent PAR model (bottom row) better understands that talking and listening actions are complementary actions, while the AR model doesn't learn this correlation. We see quantitative evidence of this in Fig.~\ref{fig:ava_2_person_classes}, with per-class mAPs for our AR vs 2-agent PAR model for 2-person action classes. Here, \textit{talk to} gets a $+4.4$ mAP gain and \textit{listen to} gets a $+7.0$ mAP gain when we train a multi-agent model. We see a significant boost on many other interaction-related action classes---for instance, \textit{kiss a person} $+8.3$ and \textit{fight/hit a person} $+5.7$ mAP---and on single-person actions, see Fig.~\ref{fig:ava_1_person_classes}.











==> _CVPR_2025__PAR__1_/sec/5_car_trajectories.tex <==
\section{Case Study 2: Multiagent Car Trajectory Prediction}
\label{sec:car_trajs}
Our second case study focuses on predicting car trajectories. Trajectory prediction requires a vehicle to be aware of other cars on the road to avoid collisions and promote cooperative behavior. This study demonstrates how our framework enables the joint modeling of multiple vehicles' movements.

\subsection{Experimental Setup}
\noindent \textbf{Dataset.} We use nuScenes~\citep{nuscenes} , inputting 2 seconds of positions to forecast vehicle positions 6 seconds ahead. Specifically, our objective is to predict the $xy$ coordinates of each agent, exclusively considering vehicles as agents. We use the \texttt{trajdata} interface~\citep{ivanovic2023trajdata} to load and visualize the data.

\noindent \textbf{Task-specific considerations.}   Instead of discretizing the $xy$ position space, we discretize the motion, resulting in discrete velocity or acceleration tokens. These integer tokens are projected to the transformer hidden dimension using the Llama token embedding layer. Inputting only these tokens results in our PAR model knowing what speed the other agents are going at, but not where they are. It is important the model has this awareness (it should know if two agents are going to collide), so our model needs to reason over this second modality of location. We implement this by passing locations relative to the agent we are predicting into a sin-cosine positional embedding (see details in Sec.~\ref{sec:appendix_car_impl_details}), which we denote a location positional encoding (LPE). The LPE is summed to our token embeddings.

We use a cross-entropy classification loss on our discrete tokens:
$\mathscr{L} = E_{y \sim p(y)}[-\log(p(\mathbf{s}^{T}_{t_{\pi}})].$  We use the standard average displacement error (ADE) and final displacement error (FDE) to evaluate our predicted trajectories. For our baselines (Sec.~\ref{sec:task-specific}), we use the closest agent at the current timestep for \textit{Multiagent NN} and \textit{Mirror}. For \textit{NN} and \textit{Multiagent NN} we use MSE as the distance metric.


\subsection{Results}
\begin{table}
% 
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
Token type & LPE & Method &  ADE $\downarrow$ & FDE $\downarrow$           \\
\midrule
Velocity  & \xmark & 1-agent AR & 1.50 & 3.64 \\
Velocity & \xmark & 3-agent PAR & 1.45 & 3.51 \\
Accleration  & \xmark   & 1-agent AR & 1.44    & 3.57  \\
Accleration  & \xmark & 3-agent PAR  & 1.40    & 3.44    \\
Accleration  & \cmark& 3-agent PAR   & \textbf{1.35} & \textbf{3.34} \\
\bottomrule
\end{tabular}
\caption{\textbf{Car trajectory prediction performance.} Using acceleration tokens and 3-agent PAR results in a stronger performance over velocity tokens and single-agent AR. Adding location via a positional encoding (LPE) further improves results. }
\label{tab:cars_locs}

% Neerja: experiment names/wandb links
% 1-agent velocity	https://wandb.ai/nthakkar/ICLR_paper_cars/runs/ccg7y19d?nw=nwusernthakkar	final_car_traj_1_agent_vel_tok_a100_full_val
% 3-agent PAR velocity	https://wandb.ai/nthakkar/ICLR_paper_cars/runs/sgi43f24	final_car_traj_3_agent_vel_tok_a100_full_val
% 1-agent acc	https://wandb.ai/nthakkar/PAR_car_traj_prediction_nuscenes/runs/k5na3q37?nw=nwusernthakkar	final_car_traj_1_agent_accl_tok_a100_full_val
% 3-agent PAR acc	https://wandb.ai/nthakkar/PAR_car_traj_prediction_nuscenes/runs/9flpua7w	final_car_traj_3_agent_accl_tok_a100_full_val
% 3-agent PAR acc + LPE	https://wandb.ai/nthakkar/PAR_car_traj_prediction_nuscenes/runs/l8fbaj7m?nw=nwusernthakkar	final_car_traj_3_agent_location_pos_embedding_sin_cos_accl_tok_relative_loc_a100_full_val

\end{table}
% 
% 
\begin{table}
\centering
\begin{tabular}{@{}lccc@{}}
\toprule
Baseline & Agents &  ADE $\downarrow$ & FDE $\downarrow$           \\
\midrule
Random Trajectory & 1  & 8.89 & 16.51      \\
NN    & 1   & 1.80 & 4.13 \\
 Multiagent NN & N & 6.40 & 12.04      \\
Mirror  & N & 11.59 & 14.93      \\
\bottomrule
\end{tabular}
\caption{\textbf{Car trajectory prediction baselines.} Nearest neighbor performs best overall, but our learned single-agent AR models outperform all baselines.}
\label{tab:cars_baselines}
\vspace{-0.25cm}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{fig/cars_qual.pdf}
    \caption{Example results from our single-agent AR model (top row) and three-agent PAR model with location positional encoding (bottom row) on nuScenes. The predicted agent's ground truth trajectory is in pink, and the predicted future in blue. For the PAR model, the other two agents' ground truth states are in green. Qualitatively, the PAR model handles situations where single-agent predictions might lead to collisions (A, B), uses other agents' behavior to better adhere to road areas (A, C) without environment data, and predicts based on the speed changes of other cars (D).}
    \label{fig:cars_qual}
    \vspace{-.6cm}
\end{figure}


We train AR and 3-agent PAR models using velocity tokens, acceleration tokens, and acceleration tokens combined with our location positional encoding. The results can be seen in Table~\ref{tab:cars_locs}. Note that the 3-agent PAR model uses the agent ID embedding and next timestep prediction.
Acceleration tokens consistently outperform velocity tokens both for agent AR and 3-agent PAR models. This could be because the vocabulary size for acceleration tokens is much smaller and therefore easier to optimize. Regardless, both ways of tokenizing result in models that outperform our baselines (see Table~\ref{tab:cars_baselines} - NN has a relatively low error on this dataset), and highlight that our framework is flexible such that a user can experiment with different ways of representing entities. For both token types, the 3-agent PAR model that is blind to location outperforms the AR model. While location information should help the model, it is possible that simply knowing whether other agents are slowing down or accelerating can help the model make better predictions.  When adding location information via the LPE to our 3-agent PAR model, we see another performance gain in ADE and FDE. 

Qualitative examples of the AR model (top row) and 3-agent location-aware PAR model (bottom row) can be seen in Figure~\ref{fig:cars_qual}. Our method uses no image or environment data (e.g., lanes) as input. However, by reasoning over multiple agents, its predictions lead to fewer collisions and better reasoning about speed changes and driveable areas based solely on other agents' behaviors.
% Note that our method does not take as input any pixels/image information, or any information about the environment such as lanes. We see evidence that when reasoning over multiple agents, our method is able to make predictions that result in fewer collisions, and better reasoning about changes in speed and what parts of the road are driveable, just based on the behaviour of other agents.







==> _CVPR_2025__PAR__1_/sec/6_hand_object.tex <==
\section{Case Study 3: Object Pose Forecasting During Hand-Object Interaction}

Our final case study explores how hand-object interaction can be leveraged for object pose estimation. We define the human hand and the interacting object as two agents, with tokens representing distinct state types. We show that our PAR framework can jointly model these agents, improving 3D translation and rotation predictions for the object. 

\begin{figure}
    \centering
    % \includegraphics[width=\linewidth]{fig/rotation_result_2_bigger_10sr_cropped_remove_whitespace.png}
    \includegraphics[width=\linewidth]{fig/new_128dim_rot.pdf}
    \vspace{-20pt}
    \caption{
    % We present a qualitative result from the validation split for the rotation prediction task.
    \textbf{Rotation forecasting qualitative result on test set.} 3D predictions are projected onto the image, isolating rotation results by showing the ground-truth translation. Incorporating the hand agent in the PAR framework (right) improves object pose prediction over object-only AR (left). %Last frame of sequence shown.
    % The projected 3D model in blue has the ground-truth translation for visualization purposes and our predicted rotation. [say how much history there was and how far into the future]
    % To account for the low dynamics between consecutive frames, we sample every 10th frame. Left (AR), the results depict the object of interest as the sole agent, while the right (2-agent PAR) demonstrates improved performance by incorporating the human hand as a second agent in the grasping interaction. \shiry{say which frame in the future are you showing}
    }
    \label{fig:ho_qual}
    % \vspace{-.5cm}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/new_128dim_tx.pdf}
    \vspace{-20pt}
    \caption{
    \textbf{Translation forecasting qualitative result on test set.} 3D predictions are projected onto the image, isolating translation results by showing the ground-truth rotation. Using the PAR framework (right) instead of AR (left) improves object pose prediction.
    }
    \label{fig:ho_qual2}
    \vspace{-.5cm}
\end{figure}

\subsection{Experimental Setup}
\noindent \textbf{Dataset.} We use the DexYCB dataset, which includes 1000 videos of 10 subjects performing object manipulation tasks with 20 distinct objects from the YCB-Video dataset. The data is split into 800 training, 40 validation, and 160 testing videos. We use one of 8 provided camera views. In each trial, subjects pick up and lift objects in randomized conditions. Labels include the object's SO(3) rotation and 3D translation, and the hand's 3D translation. We focus on predicting the object's rotation or translation.
% For this case study, we utilize the DexYCB dataset~\cite{chao2021dexycb}, which contains 1000 videos of 10 human subjects performing object manipulation tasks. Each subject picks up 20 distinct objects from the YCB-Video dataset~\cite{xiang2017posecnn}, with multiple trials conducted for each object. The dataset is divided into 800 training videos, 40 validation videos, and 160 testing videos. Although the videos are recorded from 8 RGB-D cameras, we work with a single camera view. In each trial, the subject starts in a relaxed pose with their hand by their side (often out of the camera’s view), grasps the target object, and lifts it into the air. For each subject-object pair, there are 5 trials where the object’s rotation, placement, and surrounding distractor objects are randomized. The dataset provides labels such as the object's SO(3) rotation and 3D translation, and the 3D positions of 21 hand joints in camera space. We focus on predicting either the object's rotation or translation as it is being picked up in each video.

\medskip \noindent \textbf{Task-specific considerations.} We tokenize object information in object-only experiments and both object and hand information in hand-object experiments. The object is represented as a 4D token for rotation forecasting (quaternion from SO(3) rotation) or a 3D token for translation forecasting (Euclidean coordinates). In hand-object experiments, the hand token is included with a 3D translation vector, and agent ID embeddings distinguish between the hand and object. 
Normalization is applied to all 3D translation vectors in both AR and PAR experiments; quaternions are normalized by definition and require no additional processing. 
An embedding layer projects the tokens into the transformer's hidden dimension, and another layer projects them back for prediction. 

For rotation-only forecasting, the loss is \(\mathscr{L}_{rot} = 1 - |\hat{q} \cdot q|\), where \(\hat{q}\) is the predicted quaternion and \(q\) the ground-truth quaternion. For translation-only forecasting, the loss \(\mathscr{L}_t\) is the mean squared error (MSE) between predicted and ground-truth translations. For PAR we predict relative object-to-hand translations at each frame, using the current hand position as origin, while for AR, we predict absolute object translations without considering the interacting agent. 
% For PAR, we treat the current hand translation as the origin, and predict the relative translation between the object and hand at each frame, while the hand is relative to itself at every frame. This is in contrast to AR, where we predict the absolute object translation since the interacting agent is not incorporated. 
For PAR models, we add the loss \(\mathscr{L}_h\), a MSE on hand translation. The object-only AR rotation model is optimized with \(\mathscr{L}_{rot}\), while the PAR rotation model combines \(\mathscr{L}_{rot} + \mathscr{L}_h\); similarly, the object-only translation model is trained with \(\mathscr{L}_t\), and the hand-object translation model uses \(\mathscr{L}_t + \mathscr{L}_h\). 
At inference, the first half of each video is provided, and object predictions are autoregressively generated for the second half. Translation is evaluated using MSE, while rotation is measured using geodesic distance (GEO) on SO(3).


% \medskip \noindent \textbf{Tokenization} For object-only experiments, we tokenize only the object information, while in hand-object experiments, we tokenize both the object and hand information.

% The object is represented differently depending on the task: for rotation-only prediction, we use 4-dimensional tokens derived from the quaternion representing its SO(3) rotation, while for translation-only prediction, we use 3-dimensional tokens representing the object's Euclidean coordinates. In hand-object experiments, where the hand is treated as a second agent interacting with the object, the hand is represented by a 63-dimensional vector corresponding to the Euclidean coordinates of 21 hand joints (3 joints and 1 fingertip per finger, plus 1 wrist joint). In hand-object interaction models, we also incorporate agent ID embeddings to distinguish between the hand and object.

% We use an embedding layer to project the token(s) into the transformer's hidden dimension and another to project them back into the token space for loss computation and generation. During training, we apply teacher forcing to the tokenized hand and object data. In validation, we teacher force the hand joint information while generating the object’s rotation or translation.

% %Object pose is represented as a 7D vector - 4D quaternion rotation and 3D XYZ translation. Hand pose is represented as a 63D vector of 21 XYZ joints. 

% %We learn an embedding layer to project the token into the transformers hidden dimension and another one to unproject back into the token dimension for loss computation and generation. \neerja{Since we are doing rotation and tx separately we should mention this here that we have different cases}

% %We explicitly require rotations to be valid quaternions.

% %\neerja{Explain the cases of object only, hand and object as separate tokens, and this 1.5 agent displacement thing. Currently we do loss on hand and object (but teacher force hand at inference), lay that out here.}

% \medskip \noindent \textbf{Loss} 
% For rotation-only prediction, the loss we optimize is:
% \[
%     \mathscr{L}_{rot} = 1 - |\hat{q} \cdot q|,
% \]
% where \(\hat{q}\) is the predicted quaternion representing the object's rotation in camera space, and \(q\) is the ground-truth quaternion. We apply the absolute value to account for the double-covering of quaternions in SO(3), i.e., \(q = -q\). Additionally, we ensure that the quaternions predicted by the de-projection layer are valid, meaning they have unit norm and a positive scalar component. 

% For translation-only prediction, the loss function \(\mathscr{L}_t\) is the mean squared error (MSE) between the predicted and ground-truth translations of the object. In experiments involving the hand, we also optimize for \(\mathscr{L}_h\), the MSE loss on the predicted and ground-truth hand joint positions. Additionally, we normalize the hand joints and object translations to be between 0 and 1 during training.

% The object-only rotation model is optimized with \(\mathscr{L}_{rot}\), while the hand-object rotation model uses the combined loss \(\alpha \mathscr{L}_{rot} + (1-\alpha) \mathscr{L}_h\), where $\alpha=0.33$. Similarly, the object-only translation model is trained with \(\mathscr{L}_t\), and the hand-object translation model is optimized with \(\mathscr{L}_t + \mathcal{L}_h\), where the two losses are equally weighted since they represent the same type of measurement.

% % In hand-object interaction models, we also incorporate agent ID embeddings to distinguish between the hand and object.

% \medskip

% \noindent \textbf{Metrics} During validation, we provide the first half of each video and autoregressively generate object predictions for the second half. For object translation, we evaluate performance using the MSE metric, while for object rotation, we measure error using the geodesic distance (GEO) on SO(3), which is the shortest path in radians between the predicted and ground-truth rotations. We convert the quaternions to SO(3) matrices to compute the GEO metric.

% % We use a MSE regression loss and train the model with teacher forcing - at each timestep, the previous ground-truth tokens are used in prediction. 

% % \neerja{Describe whatever metrics we settle on here - currently for rotation I think single shortest path between GT and pred rotation on the surface of the unit sphere in 3D rotation space, and MSE for translation}

% \newpage
\subsection{Results}
We compare the object-only AR models to the hand-object PAR models in Table~\ref{tab:ho_res} for the two prediction tasks. We also present the baselines described in Sec.~\ref{sec:task-specific} in Table~\ref{tab:ho_baselines}. Figures~\ref{fig:ho_qual} and~\ref{fig:ho_qual2} show qualitative results on the rotation and translation predictions, respectively. In both prediction tasks, we observe that incorporating the human hand's interaction with the object enhances accuracy: for rotation, PAR results in a relative improvement of $8.9\%$ over AR, and for translation, $41\%$. See Section~\ref{sec:app_ho_qual} for additional qualitative results with more sampled frames.
% In Figure~\ref{fig:ho_qual}, we see that the AR model (top row) achieves high-fidelity predictions early on, when much of its history still relies on ground truth data from the first half of the sequence. However, as the video progresses and the history becomes increasingly dependent on predicted object rotations, the AR model’s performance rapidly deteriorates. In contrast, our PAR model (bottom row) reasons over the 3D hand joint positions to predict the object's SO(3) rotation much more accurately. 
% Please see~\ref{app:pose} for more results on pose estimation.

\begin{table}
% \centering \footnotesize
\begin{tabular}{@{}lccc@{}}
\toprule
Type & Method &  MSE $\downarrow$ & GEO ($rad$) $\downarrow$ \\
% Type & Method &  MSE ($\times$10$^{-3}m^2$) $\downarrow$ & GEO ($rad$) $\downarrow$ \\
\midrule
Translation & 1-agent AR & 3.68 $\times$ 10$^{-3}$ & - \\
% Translation & 2-agent PAR & \textbf{3.28} & - \\
Translation & 2-agent PAR & \textbf{2.17} $\boldsymbol{\times}$ \textbf{10}$^{\boldsymbol{-3}}$ & - \\
\midrule
Rotation & 1-agent AR & - &  0.919 \\
Rotation & 2-agent PAR & - &  \textbf{0.837} \\
\bottomrule
\end{tabular}
\caption{\textbf{Test set results on DexYCB dataset.} For both rotation and translation forecasting, the 2-agent PAR model, which treats the hand as an additional agent, improves results.}
\label{tab:ho_res}
\end{table}

% \begin{table*}
% \centering \footnotesize
% \begin{tabular}{@{}lcccccc@{}}
% \toprule
% Type & Object Token & Hand Token & Ag ID Emb & Agents &  MSE ($m^2$) $\downarrow$ & GEO ($rad$) $\downarrow$           \\
% \midrule
% Translation & \cmark  & \xmark & \xmark & 1 & 2.97$\times$ 10$^{-2}$ & - \\
% Translation &  \cmark  & \cmark & \cmark & 2 & \textbf{1.90} $\boldsymbol{\times}$ \textbf{10}$^{\boldsymbol{-3}}$ & - \\
% \midrule
% Rotation & \cmark  & \xmark & \xmark & 1 & - &  0.944 \\
% Rotation & \cmark  & \cmark & \cmark & 2 & - &  \textbf{0.890} \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Test set results on DexYCB dataset.} Top two rows: translation prediction, bottom two rows: rotation prediction. In both cases, the 2-agent PAR model, which accounts hand-object interaction by integrating the hand as an additional agent, yields improved results.}
% \label{tab:ho_res}
% \end{table*}


\begin{table}
\centering \footnotesize
\begin{tabular}{@{}lcc@{}}
\toprule
Baseline &  Translation - MSE ($m^2$) $\downarrow$ & Rotation - GEO ($rad$) $\downarrow$           \\
\midrule
% Random  & 0.327 & 2.147 \\
% Random Trajectory & 1.37$\times$ 10$^{-2}$ & 2.189 \\
% NN  & 1.54$\times$ 10$^{-2}$ &  2.077\\
% Multiagent NN  & 1.31$\times$ 10$^{-2}$ & 2.268  \\
% Mirror  & 1.20$\times$ 10$^{-2}$  & N/A  \\
Random  & 0.244 & 2.196 \\
Random Trajectory & 1.60$\times$ 10$^{-2}$ & 2.146 \\
NN  & 1.69$\times$ 10$^{-2}$ &  2.179 \\
Multiagent NN  & 1.71$\times$ 10$^{-2}$ & 2.170 \\
Mirror  & 1.20$\times$ 10$^{-2}$  & -  \\
\bottomrule
\end{tabular}
\caption{\textbf{Test set results for DexYCB baselines.} We cannot provide rotation results for the Mirror baseline, because the ground-truth does not include hand rotation, only 3D translation.}
\label{tab:ho_baselines}
\end{table}










==> _CVPR_2025__PAR__1_/sec/7_conclusion.tex <==
\section{Discussion}

This work introduced the Poly-Autoregressive (PAR) framework, a unifying approach to prediction for multi-agent interactions. By applying the same transformer architecture and hyperparameters across diverse tasks, including action forecasting in social settings, trajectory prediction for autonomous vehicles, and object pose forecasting during hand-object interaction, we have demonstrated the versatility and robustness of our framework. 

Our findings underscore the crucial importance of considering the influence of multiple agents in a scene for prediction tasks. By modeling interactions, we significantly improved prediction accuracy over single-agent approaches on all three problems we considered. While we achieved promising results with a simple architecture, we have only provided a starting point that can be built upon extensively. For instance, incorporating environmental context or tokenizing pixel patches, especially as a way to relax our assumption on high-quality tracking,  are avenues for further research using PAR. It would be interesting to experiment with scaling the data and model. We do not specifically consider the relative importance of neighboring agents, which is an interesting future research direction (ex. dynamic attention mechanism).

Our PAR framework provides a simple and generalizable foundation of universal building blocks, ready for extension or refinement in future tasks. The PAR framework holds potential for advancing AI systems, enhancing prediction capabilities and enabling more accurate navigation and operation in real-world, multi-agent interactions.


\section{Acknowledgements} We thank Jane Wu, Himanshu Singh, Georgios Pavlakos, and João Carreira for useful discussions and feedback. This work was supported by ONR
MURI N00014-21-1-2801 and NSF Graduate Fellowships to NT and TS.

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
